DiscDiff: Latent Diffusion Model for DNA Sequence Generation

This paper introduces a novel framework for DNA sequence generation, comprising two key components: DiscDiff, a Latent Diffusion Model (LDM) tailored for generating discrete DNA sequences, and Absorb-Escape, a post-training algorithm designed to refine these sequences. Absorb-Escape enhances the realism of the generated sequences by correcting `round errors' inherent in the conversion process between latent and input spaces. Our approach not only sets new standards in DNA sequence generation but also demonstrates superior performance over existing diffusion models, in generating both short and long DNA sequences. Additionally, we introduce EPD-GenDNA, the first comprehensive, multi-species dataset for DNA generation, encompassing 160,000 unique sequences from 15 species. We hope this study will advance the generative modelling of DNA, with potential implications for gene therapy and protein production.

==> extra-results-refined.tex <==
\section{Additional Results}
\label{app:extra-results}
\begin{table*}[ht]
    \centering
    \begin{tabular}{
            l
            S[table-format=2.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
        }
        \toprule
                           & \multicolumn{2}{c}{Baking Yeast} & \multicolumn{2}{c}{Chicken} & \multicolumn{2}{c}{Corn}                                                                 \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        Model              & {MotifMSE $\downarrow$}          & {Div $\uparrow$}            & {MotifMSE $\downarrow$}  & {Div $\uparrow$} & {MotifMSE $\downarrow$} & {Div $\uparrow$} \\
        \midrule
        Hyena (Best)       & 0.958                            & 0.660                       & 0.956                    & 0.389            & 0.995                   & 0.546            \\
        DiscDiff (CNN-VAE) & 0.858                            & 0.523                       & 0.960                    & 0.501            & 0.983                   & 0.597            \\
        Absorb-Escape      & 0.864                            & 0.531                       & 0.910                    & 0.395            & 0                       & 0                \\
        \bottomrule
    \end{tabular}
    \caption{Conditional Generations on EPD-GenDNA-small: for human, honee, and baking yeast.}
    \label{table:conditional-extra-results-1}
\end{table*}

\begin{table*}[ht]
    \centering
    \begin{tabular}{
            l
            S[table-format=2.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
        }
        \toprule
                      & \multicolumn{2}{c}{Dog} & \multicolumn{2}{c}{Elegans} & \multicolumn{2}{c}{Fission Yeast}                                                                 \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        Model         & {MotifMSE $\downarrow$} & {Div $\uparrow$}            & {MotifMSE $\downarrow$}           & {Div $\uparrow$} & {MotifMSE $\downarrow$} & {Div $\uparrow$} \\
        \midrule
        Hyena (Large) & 0.890                   & 0.398                       & 0.930                             & 0.580            & 0.929                   & 0.641            \\
        DiscDiff      & 0.829                   & 0.544                       & 0.677                             & 0.499            & 0.860                   & 0.472            \\
        Absorb-Escape & 0.754                   & 0.438                       & 0.857                             & 0.457            & 0                       & 0                \\
        \bottomrule
    \end{tabular}
    \caption{Conditional Generations on EPD-GenDNA-small: for human, honey bee, and baking yeast.}
    \label{table:conditional-extra-results-2}
\end{table*}

\begin{table*}[ht]
    \centering
    \begin{tabular}{
            l
            S[table-format=2.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
        }
        \toprule
                      & \multicolumn{2}{c}{Fruit Fly} & \multicolumn{2}{c}{Honey Bee} & \multicolumn{2}{c}{Human}                                                                 \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        Model         & {MotifMSE $\downarrow$}       & {Div $\uparrow$}              & {MotifMSE $\downarrow$}   & {Div $\uparrow$} & {MotifMSE $\downarrow$} & {Div $\uparrow$} \\
        \midrule
        Hyena (Large) & 0.970                         & 0.725                         & 0.933                     & 0.454            & 0.922                   & 0.471            \\
        DiscDiff      & 0.813                         & 0.595                         & 0.897                     & 0.382            & 0.908                   & 0.603            \\
        Absorb-Escape & 0.937                         & 0.562                         & 0.905                     & 0.351            & 0                       & 0                \\
        \bottomrule
    \end{tabular}
    \caption{Conditional Generations on EPD-GenDNA-small: for human, honey bee, and baking yeast.}
    \label{table:conditional-extra-results-3}
\end{table*}

\begin{table*}[ht]
    \centering
    \begin{tabular}{
            l
            S[table-format=2.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
        }
        \toprule
                      & \multicolumn{2}{c}{Macaque} & \multicolumn{2}{c}{Mouse} & \multicolumn{2}{c}{Plasmodium}                                                                 \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        Model         & {MotifMSE $\downarrow$}     & {Div $\uparrow$}          & {MotifMSE $\downarrow$}        & {Div $\uparrow$} & {MotifMSE $\downarrow$} & {Div $\uparrow$} \\
        \midrule
        Hyena (Large) & 0.935                       & 0.386                     & 0.959                          & 0.566            & 0.792                   & 0.0432           \\
        DiscDiff      & 0.939                       & 0.539                     & 0.941                          & 0.626            & 0.888                   & 0.0807           \\
        Absorb-Escape & 0                           & 0                         & 0                              & 0                & 0                       & 0                \\
        \bottomrule
    \end{tabular}
    \caption{Conditional Generations on EPD-GenDNA-small: for human, honey bee, and baking yeast.}
    \label{table:conditional-extra-results-4}
\end{table*}


\begin{table*}[ht]
    \centering
    \begin{tabular}{
            l
            S[table-format=2.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
            S[table-format=3.1]
            S[table-format=1.3]
        }
        \toprule
                      & \multicolumn{2}{c}{Rat} & \multicolumn{2}{c}{Thale Cress} & \multicolumn{2}{c}{Zebrafish}                                                                 \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
        Model         & {MotifMSE $\downarrow$} & {Div $\uparrow$}                & {MotifMSE $\downarrow$}       & {Div $\uparrow$} & {MotifMSE $\downarrow$} & {Div $\uparrow$} \\
        \midrule
        Hyena (Large) & 0.972                   & 0.514                           & 0.979                         & 0.502            & 0.969                   & 0.729            \\
        DiscDiff      & 0.939                   & 0.575                           & 0.970                         & 0.492            & 0.953                   & 0.624            \\
        Absorb-Escape & 0                       & 0                               & 0.994                         & 0.403            & 0                       & 0                \\
        \bottomrule
    \end{tabular}
    \caption{Conditional Generations on EPD-GenDNA-small: for human, honey bee, and baking yeast.}
    \label{table:conditional-extra-results-5}
\end{table*}

